Security Issues in the Android Cross-Layer Architecture

The security of Android has been recently challenged by the discovery of a number of vulnerabilities involving different layers of the Android stack. We argue that such vulnerabilities are largely related to the interplay among layers composing the Android stack. Thus, we also argue that such interplay has been underestimated from a security point-of-view and a systematic analysis of the Android interplay has not been carried out yet. To this aim, in this paper we provide a simple model of the Android cross-layer interactions based on the concept of flow, as a basis for analyzing the Android interplay. In particular, our model allows us to reason about the security implications associated with the cross-layer interactions in Android, including a recently discovered vulnerability that allows a malicious application to make Android devices totally unresponsive. We used the proposed model to carry out an empirical assessment of some flows within the Android cross-layered architecture. Our experiments indicate that little control is exercised by the Android Security Framework (ASF) over cross-layer interactions in Android. In particular, we observed that the ASF lacks in discriminating the originator of a flow and sensitive security issues arise between the Android stack and the Linux kernel, thereby indicating that the attack surface of the Android platform is wider than expected.

==> ASF.tex <==
\section{Introducing the Android Security Framework}
% We should introduce the role of the Android Security Framework as a cross-layer security mechanism managing security-related aspects of layers interplay.
% In particular, we should explain the informal security policy applied to vertical interplay

\label{sec:ASF}
The Android Security Framework (ASF) consists of a set of decentralized security mechanisms spanning on all layers of the Android stack. The ASF enforces an informal and cross-layer security policy focused on the concept of \emph{permission}.

\subsection{Android Permissions}
In Android, a permission is a string expressing the ability to perform a specific operation. Permissions can be system-defined or user-defined. 
Each application statically declares the set of permissions it
requires to work properly. Such a set is generally a superset of the permissions effectively used at runtime. 
During installation of an application, the user must grant the whole set of required permissions, otherwise the installation is aborted.
Once installed, an application cannot modify such permissions. 

Each application package contains an XML file, called \emph{Android
  Manifest}, containing two types of permissions: 
\begin{itemize}
\item \textbf{declared permissions} are defined by the application
  itself and represent access rights that other applications must
  have for using its resources.  
\item \textbf{requested permissions} representing the permissions held by the application.
\end{itemize}

Since permissions specified in the manifest are static (i.e., they
cannot possibly change at runtime), they are not suited to regulate
access to resources that are dynamically defined by the application
(e.g., shared data from a content provider).  For this reason Android
APIs include special methods for dynamically (i) \emph{granting}, (ii)
\emph{revoking} and (iii) \emph{checking} access permissions.  These
methods handle per-URI permissions thereby letting the application
give temporary access privileges for some owned URI to other
applications.


\subsection{Android security policy}

The Android security policy defines restrictions on the interactions among applications and between each application and the system. The Android security policy is globally enforced by the ASF. Both the policy and the ASF strongly rely on permissions associated with the components. We detail here the security policy related to the architecture and the interactions explained in Sec. \ref{sec:architecture}.

\paragraph{Horizontal interactions.}
%\gcnote{spiegato cosi' sembra molto diverso dal modello...} \amnote{ puoi adattarlo tu che hai miglior visionedel modello? thanks.}
Horizontal interactions between components are carried out through permissions associated with intents. 
Each application can declare a list of permissions for their incoming intents.
When application $A$ sends an intent $I$ to application $B$, the platform delivers $I$ only if $A$ has the privileges (granted at installation time) requested by $B$.
Otherwise, the intent does not reach $B$ (still, it could be delivered to other recipients).
%%%%%
\paragraph{Vertical interactions.}
%\gcnote{anche questo non torna molto} \amnote{idem come sopra}
By default, an Android application can only access a limited range of
system resources.  These restrictions are implemented in different
forms.  Some capabilities are restricted by an intentional absence
APIs to access a sensitive ressource or functionality.  For instance,
there is no API that allows for the direct manipulation of the SIM
card.  In other cases, the sensitive APIs are reserved for
trusted applications and are protected through permissions.

Each API in the library layer is associated with a certain permission.
Once a component invokes an API, the privileges of the component are
checked against the permission required for the API.  If an
application attempts to invoke an API without having the proper
privileges, a security exception is thrown and the invocation fails.

\paragraph{Linux layer and IPC.}
The Android platform takes advantage of the Linux user-based access
control model as a means to identify and isolate application
resources. The Android system assigns a unique user ID (UID) to each
Android application and runs it as that user in a separate Linux
process.  This sets up a kernel-level \emph{Application Sandbox}. This
approach uses the native Linux isolation for users to implement a
security policy that avoids direct communications among Android
applications by forcing all their interactions to rely upon the IPC
system.  However, such a policy does not prevent a Linux process
(running an application) from communicating through one of the native
UNIX mechanisms such as sockets or files. Notice that the Linux
permissions apply on such channels.

The previous analysis shows the cross-layer nature of Android Security
policy. The ASF is distributed and involves distinct security-relevant
aspects (from UID and GID at Linux layer to human-readable and high
level Android permissions). Assessing the effectiveness of all the
security mechanisms and their interplay is difficult due to such
heterogeneity and the lack of a detailed and comprehensive model of
the security-relevant aspects of Android.

==> macro.tex <==
\newcounter{fixcountermargin}
\setcounter{fixcountermargin}{0}
\newcounter{fixcounter}
\setcounter{fixcounter}{0}

\newcommand{\fix}[1]{$^{\addtocounter{fixcountermargin}{1}[\arabic{fixcountermargin}]
}$\marginpar{\small\raggedleft$^{[\arabic{fixcountermargin}]}$#1}}


\newcommand{\fixfootnote}[1]{$^{\{\textsf{FIX}\addtocounter{fixcounter}{1}}$\footnote[\arabic{fixcounter}]{{\textsf{FIX.} #1}}$^{\}}$}
% \newcommand{\fixfootnote}[1]{}
%\newcommand{\fixfootnoteavispa}[1]{$^{[\textsf{FIX}\addtocounter{fixcounteravispa}{1}}$\footnote[\arabic{fixcounteravispa}]{{\textsf{FIX AVISPA.} #1}}$^{]}$}

\newcommand{\fixn}[2]{\fixfootnote{\textbf{#1:} #2}}
%\newcommand{\fixn}[2]{}

\newcommand{\unused}[1]{}
% \newcommand{\SignedBy}[2]{\{#1\}_{\text{K}^{-1}_{#2}}}

\newcommand{\aslanpp}{ASLan{\small ++}}
\newcommand{\aslan}{ASLan}
\DeclareMathOperator{\imp}{\Rightarrow}

\newcommand{\Lhs}{{L}}                  %% Rewrite rule: instance of the LHS
%%\newcommand{\L}{{L(x)\sigma}}
\newcommand{\Rhs}{{R}}                    %% Rewrite rule: instance of the LHS
\newcommand{\rw}[1]{\xrightarrow[]{#1}}
\newcommand{\ifs}[1]{{\mathtt{#1}}}
\newcommand{\w}[1]{\mathtt{state}_{#1}}
\newcommand{\den}[1]{{[\![#1]\!]}}
\newcommand{\pgm}[1]{{\lceil#1\rceil}}
\newcommand{\closure}[1]{{\downarrow\!\!{#1}}}

\DeclareMathOperator{\ak}{\mathtt{ak}}
\DeclareMathOperator{\hasvc}{\mathit{has\_vc}} %[RC] Added
\DeclareMathOperator{\hasat}{\mathit{has\_at}} %[RC] Added
\DeclareMathOperator{\ik}{\mathtt{ik}}
\DeclareMathOperator{\intruder}{\mathtt{i}}
\DeclareMathOperator{\state}{\mathtt{state}}
\DeclareMathOperator{\sent}{\mathtt{sent}}
\DeclareMathOperator{\rcvd}{\mathtt{rcvd}}
\DeclareMathOperator{\net}{\mathtt{net}}
\DeclareMathOperator{\iswr}{\mathtt{writable}}
\DeclareMathOperator{\isrd}{\mathtt{readable}}
\DeclareMathOperator{\islossy}{\mathtt{lossy}}
\DeclareMathOperator{\counter}{\mathtt{c}}
\DeclareMathOperator{\contains}{\mathtt{contains}}
\DeclareMathOperator{\dom}{dom}

\DeclareMathOperator{\somefuture}{\mathbf{F}}
\DeclareMathOperator{\onefuture}{\mathbf{X}}
\DeclareMathOperator{\allpast}{\mathbf{H}}
\DeclareMathOperator{\once}{\mathbf{O}}
\DeclareMathOperator{\onepast}{{\mathtt{Y}}}
\DeclareMathOperator{\always}{\mathbf{G}}
\DeclareMathOperator{\release}{{\mathbf{R}}}
\DeclareMathOperator{\until}{{\mathbf{U}}}
\DeclareMathOperator{\f}{f}
\DeclareMathOperator{\g}{g}
\DeclareMathOperator{\rwapp}{app}

\DeclareMathOperator{\pre}{pre}
\DeclareMathOperator{\add}{add}
\DeclareMathOperator{\del}{del}

\DeclareMathOperator{\lhs}{lhs}
\DeclareMathOperator{\rhs}{rhs}

\DeclareMathOperator{\dd}{\centerdot}
\DeclareMathOperator{\ifscond}{\mathtt{\&}}

\newcommand{\pipmv}[1]{\mathit{#1}}
\newcommand{\metafunc}[1]{{\emph{#1\,}}}

\newcommand{\makeprogress}{{\mathit{progress}}}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

